Let's Make a Splan: Risk-Aware Trajectory Optimization in a Normalized Gaussian Splat

Neural Radiance Fields and Gaussian Splatting have recently transformed computer vision by enabling photo-realistic representations of complex scenes. However, they have seen limited application in real-world robotics tasks such as trajectory optimization. This is due to the difficulty in reasoning about collisions in radiance models and the computational complexity associated with operating in dense models. This paper addresses these challenges by proposing SPLANNING, a risk-aware trajectory optimizer operating in a Gaussian Splatting model. This paper first derives a method to rigorously upper-bound the probability of collision between a robot and a radiance field. Then, this paper introduces a normalized reformulation of Gaussian Splatting that enables efficient computation of this collision bound. Finally, this paper presents a method to optimize trajectories that avoid collisions in a Gaussian Splat. Experiments show that SPLANNING outperforms state-of-the-art methods in generating collision-free trajectories in cluttered environments. The proposed system is also tested on a real-world robot manipulator. A project page is available at https://roahmlab.github.io/splanning.

==> appendices/05_normalized_3DGS_original.tex <==
\section{Normalized 3D Gaussian Splatting}\label{app:normalized-3DGS}

\newcommand{\rorig}{r_o}
\newcommand{\rdir}{r_d}
\let\temp\phi
\let\phi\varphi
\let\varphi\temp
\let\bar\overline
\newcommand{\loss}{\mathcal{L}}
\newcommand{\rC}{\mathcal{C}} % rendered color
\newcommand{\rD}{\mathcal{D}} % rendered color
\newcommand{\pC}{c} % color as a property
\newcommand{\tn}{\Tilde{n}} % |J| * n
\newcommand{\gauss}[2]{\exp\left(-\frac{1}{2}\norm{#1}_{#2}^2\right)}
\newcommand{\Du}{\Delta u}
\newcommand{\rbar}[1]{\left.#1\right|}
\newcommand{\part}[2]{\frac{\partial #1}{\partial #2}}

This appendix provides a detailed derivation of the rasterization process of a normalized 3D Gaussian Splat and the computation of its derivative with respect to the splatting parameters.
In order to remain consistent with the splatting literature, the notation in this section is self-contained and distinct from the notation used in the rest of the document.
In practice, the reference implementation of the original 3D Gaussian Splatting method \cite{kerbl20233d} was modified to include normalization in both the forward and backward pass.

\subsection{Radiance Field Preliminaries}
First, we re-state the definition of a radiance field.
A radiance field models the image formation process by approximating a five-dimensional function that maps from a point and viewing directions to the differential opacity $\sigma: \R^3 \to \R$ and the color $\pC: \R^3 \times S^2 \to \R^3$.
Intuitively, $\sigma$ represents the likelihood that a particle traveling along a ray will stop when it collides with an individual point in space.
Under a radiance field model, an image is rendered by considering separately the ray that intersects each pixel.
Consider a ray $r(s) : \R \to \R^3$.
We define an additional quantity, the \textit{transmittance}, which defines the probability that a particle traveling along ray $r$ from $s=a$ to $s=b$ will experience a collision. 
This transmittance, denoted as $\T_a^b[r]$, is computed by

\begin{equation}\label{eq:app-transmittance}
    \T_a^b[r] = \exp\left(-\int_a^b \sigma(r(s))ds\right)
\end{equation}
Equivalently, $\T_a^b[r]$ may be interpreted by considering a light source aligned with ray $r$ and located at $s=a$.
Then $\T_a^b[r]$ is the proportion of light that remains by point $s=b$.

From the transmittance, the expected color of the pixel corresponding to ray $r$ can be computed as
\begin{equation}\label{eq:rendering-equation}
    \rC[r] = \int_{z_n}^{z_f} \pC(r(s), \rdir)\sigma(r(s)) T_{z_n}^s[r]ds
\end{equation}
where $z_n, z_f$ are the near and far clipping planes. 
The expected depth can be analogously computed as
\begin{equation}\label{eq:depth-rendering-equation}
    \rD[r] = \int_{z_n}^{z_f} s \cdot \sigma(r(s)) T_{z_n}^s[r]ds
\end{equation}

\subsection{Summary of Splatting Methods}
This section summarizes splatting methods, while the rest of the Appendix provides a detailed derivation of Normalized 3DGS.
We refer the interested reader to \cite{zwicker2002ewa} for a more comprehensive treatment of splatting-based rendering.
In a splatting framework, 3D Gaussian functions are used as a basis set to approximate $\sigma$ and $\pC$.
We call each Gaussian function a 3D reconstruction kernel $\kappa(x)$ in world coordinates.
Then, each 3D function $\kappa(x)$ is transformed into a coordinate system aligned with each camera ray.
This yields a 3D reconstruction kernel $\kappa'(x)$ in ray coordinates.
Next, each kernel is integrated along the depth dimension of the ray to yield a 2D image-space reconstruction kernel $q(x)$.
Finally, the 2D kernels are queried at the center of each pixel and blended to compute the final pixel color.

\subsection{Representation}

Let $n_G$ 3D Gaussian density functions be reconstruction kernels to represent the scene.
Let each function parameterized by mean $\mu_k$ and covariance $\Sigma_k$, both expressed in world coordinates.
Denote $S_k$ = $\Sigma_k^{-1}$. 
Then, the 3D reconstruction kernel is given by the 3D Gaussian density
\begin{equation}\label{eq:gaussian-density}
    G_k(x) = \frac{1}{\sqrt{(2\pi)^3\det{\Sigma_k}}}\gauss{x - \mu_k}{S_k}
\end{equation}
where the represented norm is the Mahalanobis distance.
For notational simplicity, we denote
\begin{equation}\label{eq:normalizing_const}
    n_k = \frac{1}{\sqrt{(2\pi)^3\det{\Sigma_k}}}
\end{equation}
as the normalizing constant of the Gaussian.
Finally, the differential opacity $\sigma$ at a point $x$ is given by
\begin{align}\label{eq:gaussian-sigma-basis}
\begin{split}
    \sigma(x) &= \sum_{k=1}^{n_G} w_k G_k(x) \\
    &= w_k n_k \gauss{x - \mu_k}{S_k}
\end{split}
\end{align}
where $w_k \in \R^+$ are positive weights.

Additionally, assume without loss of generality that the Gaussian carries with it a viewpoint-independent color $\pC_k \in \R^3$.
This assumption is made without loss of generality because, in practice, a viewpoint-dependent color may be converted to a constant color once a viewpoint is selected.
Additionally, we assume the covariance $\Sigma_k$ is provided.
In implementation, $\Sigma_k$ is parameterized by its Eigendecomposition; this detail is omitted for brevity.

% In summary, the parameters of each Gaussian $G_k$ in the scene representation are:
% \begin{itemize}[nosep]
%     \item $\Sigma_k \in \R^{3 \times 3}$, covariance of the Gaussian.
%     \item $\mu_k \in \R^3$, the mean of the Gaussian.
%     \item $\pC_k \in \R^3$, the color of each Gaussian.
%     \item $w_k \in \R^+$, the weight of each Gaussian.
% \end{itemize}in P
In summary, the parameters of each Gaussian $G_k$ in the scene representation are the mean of the Gaussian $\mu_k \in \R^3$; the covariance of the Gaussian $\Sigma_k \in \R^{3 \times 3}$; the color of each Gaussian $\pC_k \in \R^3$; and the weight of each Gaussian $w_k \in \R^+$.


\subsection{Integration of an Individual Gaussian}\label{sec:integrating-gaussians}

During the forward pass, each Gaussian is transformed into a coordinate frame aligned with each camera ray, which reduces the integration problem to a set of Gaussian marginalizations.

This section closely follows Section 6.2 of \cite{zwicker2002ewa}, with slight modifications for coordinate systems and notation.
Further, \cite{ye2023gsplatmath} provides a similar derivation for the more standard un-normalized 3D Gaussian Splatting.
We consider the integration of an individual reconstruction kernel $\kappa_k(x) = G_k(x)$ along an individual camera ray.
Let $G_k$ have mean $\mu_k$ and covariance $\Sigma_k$ expressed in world coordinates.
Denote the homogenous $SE(3)$ transformation from world coordinates to camera coordinates as
\begin{equation}
    T_{CW} = \begin{bmatrix}
        R_{CW} & d_{CW} \\
        0 & 1
    \end{bmatrix},
\end{equation}
where $R_{CW} \in SO(3)$ is a rotation matrix and $d_{CW} \in \R^3$ is a translation vector.

Consider transforming a point $x \in \R^3$ to image coordinates.
First, we transform it to camera coordinates by $t = \phi(x) = R_{CW}x + d_{CW}$, where $t \in \R^3$.
Denote the mean in camera coordinates as $\mu_k^t = \phi(\mu_k)$.
Then, points are transformed to a ray coordinate system via a projective transformation. 
We use the standard projection matrix from camera to clip space, defined as
\begin{equation}
    P = \begin{bmatrix}
        2f_x/W & 0 & 0 & 0\\
        0 & 2f_y/H & 0 & 0\\
        0 & 0 & \frac{z_f+z_n}{z_f-z_n} & -2\frac{z_fz_n}{z_f-z_n}\\
        0 & 0 & 1 & 0
    \end{bmatrix}.
\end{equation}
We simultaneously convert the first two components to pixel units via the camera's focal lengths $f_x$ and $f_y$, image size $(W, H)$, and principal point $(c_x, c_y)$: 

\begin{align}
    \varphi(t) &= 
        \begin{bmatrix}
            \frac{W P\cdot t_x}{2P\cdot t_w} + 0.5 + c_x \\
            \frac{H P\cdot t_y}{2P\cdot t_w} + 0.5 + c_y \\
            \norm{t}
        \end{bmatrix}\\
        &= \begin{bmatrix}
        f_xt_x/t_z + 0.5 + c_x \\
        f_yt_y/t_z + 0.5 + c_y \\
        \norm{t}
    \end{bmatrix}.\label{eq:image-coordinates}
\end{align}
Since the transformation \eqref{eq:image-coordinates} is not affine, it is approximated with a first-order Taylor approximation around $\mu^t$:
\begin{equation}
    \varphi_{\mu_k^t}(t) = \varphi(\mu_k^t) + J_k(t - \mu_k^t)
\end{equation}
where $J_k$ is the Jacobian of the transformation in \eqref{eq:image-coordinates}. In particular,
\begin{equation}\label{eq:J}
    J_k = \begin{bmatrix}
        f_x/\mu^t_{k,z} & 0 & -f_x\mu^t_{k,x}/{\mu^t_{k,z}}^2 \\
        0 & f_y/\mu^t_{k,z} & -f_y\mu^t_{k,y}/{\mu^t_{k,z}}^2 \\
        \mu^t_{k,x}/\norm{t_k}& \mu^t_{k,y}/\norm{\mu^t_{k}} & \mu^t_{k,z}/\norm{\mu^t_k}
    \end{bmatrix}
\end{equation}

Applying these transformations results in a ray-space reconstruction kernel given by
\begin{align}\label{eq:ray-space-kernel}
    \kappa'(u) &= \det{R_{CW}}\det{J_k}G_k'(u) \\
    \mu_k' &= \varphi(\phi(\mu_k)) \\
    \Sigma_k' &= J_kR_{CW}\Sigma R^\top _{CW}J_k^\top \label{eq:sigmaprime}
\end{align}
where $G_k'$ is a Gaussian density with mean $\mu_k'$ and covariance $\Sigma_k'$.
We refer the interested reader to \cite[Section 6.2.2]{zwicker2002ewa} for a detailed justification of the above.
Note that $R_{CW}$ is a rotation matrix, so its determinant $\det{R_{CW}} =1$ will be excluded moving forward. 

Finally, the image-space 2D reconstruction kernel is computed by marginalizing the third dimension of $\kappa'$.
As demonstrated in \cite[Section 6.2.3]{zwicker2002ewa}, this is equivalent to
\begin{equation}\label{eq:2d-reconstruction-kernel}
    q_k(\hat{u}) = \det{J_k}\hat{G}_k'(\hat{u})
\end{equation}
where $\hat{u} \in \R^2$ indicates a point on the image plane in pixel coordinates, and $\hat{G}'$ is a 2D Gaussian function with mean $\hat{\mu}_k'$ and covariance $\hat{\Sigma}'_k$ constructed by the first two rows (and columns) of the corresponding parameters of $G'_k$. We will denote the normalizing constant of $\hat{G}_k$ as $\hat{n}_k$.

\subsection{Compositing the Integrated Gaussians}
The per-Gaussian integration yields 2D reconstruction kernels which are then queried and blended onto the image plane to complete the rasterization.
In this description, we omit implementation-specific details of rasterization, including how the pixels are split into tiles, which Gaussians are included for rasterization in which tiles, and how the Gaussians are sorted.
Instead, we focus only on mathematically relevant aspects of the process, and assume without loss of generality that every Gaussian is included for rasterization in every pixel.

With this assumption, we may write a rasterization form of \eqref{eq:rendering-equation} to compute the color of a pixel with 2D coordinates $\hat{u}$
\begin{equation}\label{eq:rasterization}
    \rC(\hat{u}) = \sum_{k=1}^{n_G} w_k \pC_k q_k(\hat{u}) \prod_{j=1}^{k-1}\left(1 - w_jq_j(\hat{u}))\right).
\end{equation}
Zwicker et. al. \cite{zwicker2002ewa} provides a more thorough derivation of the above.
We may recognize the product on the right-hand-side as the transmittance $\T_k(\hat{u})$ and define $\alpha_k(\hat{u}) = w_kq_k(\hat{u})$ to simplify \eqref{eq:rasterization} to 
\begin{equation}\label{eq:rasterization-simple}
    \rC(\hat{u}) = \sum_{k=1}^{n_G}\alpha_k(\hat{u}) \pC_k \T_k(\hat{u}).
\end{equation}
In practice, the above is implemented by iterating over the Gaussian functions front-to-back once per pixel, and keeping running track of the product on the right-hand-side.
The depth is analogously rendered by
\begin{equation}\label{eq:depth-rasterization}
    \rD(\hat{u}) = \sum_{k=1}^{n_G}\alpha_k(\hat{u}) \mu^t_{k,z} \T_k(\hat{u})
\end{equation}
where $\mu^t_{k,z}$ denotes the $z$ component of the $k^{th}$ mean in the camera's frame.

\subsection{Backward Pass}
In this section, we derive the gradient of the rendered color $\rC(\hat{u})$ and depth $\rD(\hat{u})$ of the pixel $\hat{u}$ with respect to the parameters of the Gaussian Splat.
We derive the gradient for a single pixel $\hat{u} \in \R^2$; in practice, the total gradient for each Gaussian parameter results from the summation of the below derivation over all the pixels.

We may write the contribution of the $k^{\text{th}}$ Gaussian to $\rC(\hat{u})$ and $\rD(\hat{u})$ as
\begin{align}\label{eq:start-of-backward}
    \rC_k(\hat{u}) = \alpha_k(\hat{u})\pC_k\T_k(\hat{u})\\
    \rD_k(\hat{u}) = \alpha_k(\hat{u})\mu^t_{k,z}\T_k(\hat{u})
\end{align}
Next, \eqref{eq:rasterization-simple} and \eqref{eq:depth-rasterization} give that
\begin{equation}
    \part{\rC(\hat{u})}{\rC_k(\hat{u})} = \part{\rD(\hat{u})}{\rD_k(\hat{u})} = 1.
\end{equation}
Thus, we generally consider the impact of a single Gaussian on the rendered color and depth.
The dependence of variables on $\hat{u}$ will be omitted for notational simplicity.
Finally, we assume that an arbitrary loss function $\L$ is used in training.
Further, we assume that  the backward pass of the optimization provides the gradients of the loss function with respect to the rendered depth $\rD_k$ and the rendered color $\rC_k$.
We denote these input gradients as
\begin{equation*}
    \part{\L}{\rD_k}, \part{\L}{\rC_k}
\end{equation*}
respectively.
The remainder of this document specifies how to propagate these given gradients to the parameters of the Gaussian Splat.

\subsection{Gradient of the Render Process}
We begin at the end of the forward pass by differentiating \eqref{eq:rasterization-simple}, in which the integrated 2D Gaussians are composited to form pixels.
The input to the forward render pass are the 2D means $\hat{\mu}'_k$, inverses of the 2D covariances $\hat{S}'_k$, RGB colors $c_k$, normalizing constants $n_k$, and the determinant of the projection operation $\det{J_k}$. For convenience, denote
\begin{equation}
    \tn_k = \det{J_k}\hat{n}_k.
\end{equation}
The backwards render pass propagates gradients with respect to $\hat{\mu}'_k$, $\hat{S}'_k$, $c_k$, and $\tn_k$.

In implementation, we iterate over the Gaussians back-to-front.
During the forward pass, we store the final transmittance $\T_{n_G}$ for each pixel such that during the backward pass, we may iteratively compute 
\begin{equation}
    \T_{k-1} = \frac{\T_{k}}{1 - \alpha_{k-1}}. 
\end{equation}

Starting with the color parameters $c_k$, we find
\begin{align}\label{eq:color-grad}
    \part{\rC_k}{\pC_k} &= \alpha_k \T_k.\\
    \part{\L}{\pC_k} &= \alpha_k \T_k \cdot \part{\L}{\rC_k}.
\end{align}
This completes the gradient with respect to the color parameter $c_k$.

Similarly, we may differentiate \eqref{eq:depth-rasterization} with respect to the input depth of the Gaussian, $\mu^t_{k,z}$:
\begin{align}\label{eq:depth-grad}
    \part{\rD_k}{\mu^t_{k,z}} &= \alpha_k \T_k\\
    \rbar{\part{\L}{\mu^t_{k,z}}}_{\rD_k} &= \alpha_k \T_k \cdot \part{L}{\rD_k},\end{align}
where the bottom term denotes the contribution to the gradient due to the rendered depth.
We will put this term aside and revisit it later in the backward pass. 

Next, we consider the derivative of the rendered color with respect to $\alpha_k$.
\begin{align}\label{eq:dck_dalpha}
    \part{\rC_k}{\alpha_k} &= \pC_k \T_k.
\end{align}
We additionally must consider the impact of $\alpha_k$ on all future colors, which we denote 
\begin{align}\label{eq:barc_k}
    \bar{\rC}_k = \sum_{j = k+1}^{n_G} c_j \alpha_j \T_j.
\end{align}
Differentiating with respect to $\alpha_k$ gives
\begin{align}
    \part{\bar{\rC}_k}{\alpha_k} &= -\frac{\bar{\rC}_k}{1-\alpha_k} \\
    \rbar{\part{\loss}{\alpha_k}}_{\rC} &= \part{\L}{\rC} \left(\pC_k\T_k - \frac{\bar{\rC}_k}{1-\alpha_k} \right)
\end{align}
Note that $\bar{\rC}_k$ may also be computed iteratively backwards beginning with $\bar{\rC}_{n_G} = 0$. Analogously, 
\begin{align}\label{eq:dDk_dalpha}
    \bar{\rD}_k &= \sum_{j=k+1}^{n_G} \mu^t_{j,z}\alpha_j\T_j \\
    \rbar{\part{\loss}{\alpha_k}}_{\rD} &= \part{\L}{\rD_k} \left(\mu^t_{k,z}\T_k - \frac{\bar{\rD}_k}{1-\alpha_k} \right)
\end{align}
This allows
\begin{equation}\label{eq:dL_dalphak}
    \part{\L}{\alpha_k} = \rbar{\part{\L}{\alpha_k}}_{\rC} + \rbar{\part{\L}{\alpha_k}}_{\rD}
\end{equation}

We now continue to backpropagate through $\alpha_k$. Recall that
\begin{equation}\label{eq:alpha-reminder}
    \alpha_k = w_k \tn_k\gauss{\hat{u}-\hat{\mu}'_k}{\hat{S}'_k}.
\end{equation}
Since it will be frequently used, denote
\begin{equation}
    \rho_k := \gauss{\hat{u}-\hat{\mu}'_k}{\hat{S}'_k}.
\end{equation}
From \eqref{eq:alpha-reminder}, we find
\begin{equation}
    \part{\alpha_k}{w_k} = \tn_k \rho_k,\quad
    \part{\alpha_k}{\tn_k} = w_k \rho_k,\quad
    \part{\alpha_k}{\rho_k} = w_k \tn_k,
\end{equation}
which gives
\begin{align}
    \part{\L}{w_k} &= \part{\L}{\alpha_k}\tn_k \rho_k \label{eq:dL_dwk} \\
    \part{\L}{\tn_k} &= \part{\L}{\alpha_k}w_k \rho_k \label{eq:dL_dtnk} \\
    \part{\L}{\rho_k} &= \part{\L}{\alpha_k}w_k \tn_k \label{eq:dL_drhok}.
\end{align}
The second equation \eqref{eq:dL_dtnk} completes the backward pass of the render process with respect to the input $\tn_k$.

We now continue to backpropagate through $\rho_k$.
Denote 
\begin{equation}
    \Du_k = \hat{u} - \hat{\mu}'_k.
\end{equation}
Then we may compute the partial derivative of $\rho_k$ with respect to the 2D mean $\hat{\mu}'_k$ via
\begin{equation}
    \part{\rho_k}{\Du_k} = -\rho_k\hat{S}'\Du_k
\end{equation}
and
\begin{align}\label{eq:dL_dmuhatprime}
\begin{split}
    \part{\L}{\hat{\mu}_k'} &= \part{\L}{\alpha_k}\cdot\part{\alpha_k}{\rho_k}\cdot\part{\rho_k}{\Du_k}\cdot\part{\Du_k}{\hat{\mu}'_k} \\
    &= -\part{\L}{\alpha_k}\cdot\part{\alpha_k}{\rho_k}\cdot\part{\rho_k}{\Du_k}_.
\end{split}
\end{align}
This completes the gradient of the loss with respect to the 2D mean.

We may also compute the partial derivative of $\rho_k$ with respect to the elements of $\hat{S}_k'$, the inverse of the 2D covariance, via
\begin{equation}
    \part{\rho_k}{\hat{S}'_k} = \frac{\rho_k}{2}\Du_k^\top \Du_k,
\end{equation}
which allows
\begin{equation}\label{eq:dL_dconic}
    \part{\L}{\hat{S}_k'} = \part{\L}{\alpha_k}\cdot\part{\alpha_k}{\rho_k}\cdot\part{\rho_k}{\hat{S}_k}.
\end{equation}
This completes the gradient of the rendered color with respect to the inverse 2D covariance.

We have now computed the gradients of $\L$ with respect to $\hat{\mu}'_k$, $\hat{S}'_k$, $c_k$, and $\tn_k$, which completes the backward pass of the rendering function.

\subsection{Gradients of the Gaussian Integration}
The second step of the backward pass is to propagate the gradients through the coordinate transformations and marginalization described in Section~\ref{sec:integrating-gaussians}.
We differentiate the outputs of the integration step, which are $\hat{\mu}'_k$, $\hat{S}'_k$, and $\tn_k$.

\paragraph{Derivatives of $\tn_k$}
We begin by considering the derivatives of $\tn_k$. Recall that 
\begin{equation}\label{eq:tnk-reminder}
    \tn_k = \frac{\det{J_k}}{2\pi\sqrt{\det{\hat{\Sigma}'_k}}}.
\end{equation}
We start by considering the derivative of $\tn_k$ with respect to the elements of $J_k$. Recall that $J_k$ appears not just in the numerator of \eqref{eq:tnk-reminder}, but also in the definition of $\hat{\Sigma}'_k$.
First, from \cite[Eq. 49]{matrixcookbook}, we have the derivative of $\tn_k$ with respect to $J_k$ due to the inclusion of $\det{J_k}$ is
\begin{equation}\label{eq:dtnk_djkdetj}
    \rbar{\part{\tn_k}{J_k}}_{\det{J_k}} = \frac{\det{J_k}J_k^{-T}}{\sqrt{2\pi\det{\hat{\Sigma}'_k}}}.
\end{equation}
We now pause dealing with $J_k$, and turn our attention to the $\det{\Sigma'_k}$ term in the denominator of \eqref{eq:tnk-reminder}. 
By the same identity from \cite[49]{matrixcookbook},
\begin{equation}
    \part{\tn_k}{\hat{\Sigma}'_k} =\frac{\det{J_k}\left(\hat{\Sigma}'_k\right)^{-T}}{4\pi\sqrt{\det{\hat{\Sigma'_k}}}}.
\end{equation}
Continuing,
\begin{align}
    \part{\tn_k}{\Sigma'_k} &= \begin{bmatrix}
         \part{\tn_k}{\hat{\Sigma}'_k} & 0 \\
         0 & 0
    \end{bmatrix}\\
    \rbar{\part{\L}{\Sigma'_k}}_{\tn_k} &= \part{\L}{\tn_k}\cdot\part{\tn_k}{\Sigma'_k}
    % \part{\tn_k}{\Sigma_k} &= R_{CW}^\top J_k^\top \part{\tn_k}{\Sigma'_k}J_kR_{CW},\label{eq:dtnk_dsigmak}
\end{align}
where the second term denotes the contribution to the partial derivative by $\tn_k$.
% where the second equation follows from the definition of $\Sigma'_k$ in \eqref{eq:sigmaprime}.

\paragraph{Derivatives of $\hat{S}'_k$}
Given the derivative $\frac{\partial \L}{\partial \hat{S}'_k}$ computed in \eqref{eq:dL_dconic}, we may repeatedly apply \cite[Eq.~60]{matrixcookbook} to find the partial derivatives with respect to $\hat{\Sigma}'_k = \left(\hat{S}'_k\right)^{-1}$.
The results are omitted for brevity.

From this, it is trivial to apply the chain rule element-wise to obtain the partial derivatives of $\L$ with respect to $\hat{\Sigma}'_k$ due to $\hat{S'}_k$, which we denote
\begin{equation*}
    \rbar{\part{\L}{\hat{\Sigma}'_k}}_{\hat{S}'_k}
\end{equation*}
Continuing, we observe
\begin{align}
    \rbar{\part{\L}{\Sigma'_k}}_{\hat{S}'_k} &= \begin{bmatrix}
         \rbar{\part{\L}{\hat{\Sigma}'_k}}_{\hat{S}'_k} & 0 \\
         0 & 0
    \end{bmatrix}.
\end{align}
Finally, we arrive at the derivative of the loss $\L$ with respect to the transformed covariance $\Sigma'_k$
\begin{equation}
    \part{\L}{\Sigma'_k} = \rbar{\part{\L}{\Sigma'_k}}_{\hat{S}'_k} + \rbar{\part{\L}{\Sigma'_k}}_{\tn_k}
\end{equation}
We conclude the derivatives with respect to $\Sigma_k$ by transforming this back to the source coordinate system by
\begin{equation}
    \part{\L}{\Sigma_k} = R_{CW}^\top J_k^\top \part{\L}{\Sigma'_k}J_kR_{CW}.
\end{equation}

Now, we continue to backpropagate the gradients with respect to $J_k$. Denote $T_k = J_kR_{CW}$. Then
\begin{align}
    \part{\L}{T_k} &= \left(\part{\L}{\Sigma'_k}^\top + \part{\L}{\Sigma'_k}\right)T_k\Sigma_k \label{eq:dck_dtk}\\
    \part{T_k}{J_k} &= R_{CW}.\label{eq:dtk_djk}
\end{align}
This brings us to
\begin{equation}
    \part{\L}{J_k} = \part{\L}{\tn_k}\rbar{\part{\tn_k}{J_k}}_{\det{J_k}} + \part{\L}{T_k}\part{T_k}{J_k}
\end{equation}
where the first term is given by \eqref{eq:dL_dtnk} and \eqref{eq:dtnk_djkdetj}, and the second is given by \eqref{eq:dck_dtk} and \eqref{eq:dtk_djk}.
$J_k$ depends on $\mu^t_k$, so we continue to backpropagate.
\begin{align}
    \part{\L}{\mu^t_k} &= \begin{bmatrix}\sum_{i=1}^3\sum_{j=1}^3 \part{\L}{J_{k,(i,j)}}\part{J_{k,(i,j)}}{\mu^t_{k,n}}\end{bmatrix}^\top_{n=\{1,2,3\}}\label{eq:dL_dmukt} \\
    &\quad + \begin{bmatrix} 0 & 0 & \rbar{\part{\L}{\mu^t_{k,z}}}_{\rD_k}\end{bmatrix}^\top\nonumber,
\end{align}
where $J_{k, (i,j)}$ denotes the $(i,j)$ entry of $J_k$. In practice, each term in \eqref{eq:dL_dmukt} was computed symbolically, and the result is omitted here for brevity.
Finally, we arrive at the gradient of $\L$ with respect to $\mu_k$ due to the contribution from $J_k$ as
\begin{equation}
    \rbar{\part{\L}{\mu_k}}_{J_k} = R_{CW}^\top\part{\L}{\mu^t_k}
\end{equation}

\paragraph{Gradient of of $\hat{\mu}_k'$}
The final term to differentiate is $\hat{\mu}_k'$.
Immediately, we find that
\begin{align}
    \part{\hat{\mu}_k'}{\mu_k} &= \part{\hat{\mu}'_k}{\mu'_k}\cdot  \part{\mu_k'}{\mu^t_k} \cdot \part{\mu^t_k}{\mu_k} \\
    &= \begin{bmatrix}
        1 & 0 & 0 \\
        0 & 1 & 0
    \end{bmatrix} \cdot J_k \cdot R_{CW}.
\end{align}
This may be used to compute
\begin{equation}
    \rbar{\part{\L}{\mu_k}}_{\hat{\mu}'_k} = \part{\L}{\hat{\mu}'_k}\cdot \part{\hat{\mu}_k'}{\mu_k}.
\end{equation}
This gives the final gradient,
\begin{equation}
    \part{\L}{\mu_k} = \rbar{\part{\L}{\mu_k}}_{\hat{\mu}'_k} + \rbar{\part{\L}{\mu_k}}_{J_k}
\end{equation}

The above gradients were incorporated into a PyTorch automatic differentiation framework, based largely on the reference implementation provided by \cite{kerbl20233d}.

==> appendices/06_additional_experiments.tex <==
\section{Additional Experiments}
% \iftoggle{abbreviate}{}{
\input{tables/normalized_3dgs}
\input{tables/norm_3dgs_depth}
% }
This section assesses the effectiveness of \methodname's by evaluating Normalized 3DGS reconstructions.

\subsection{Normalized 3DGS Evaluation}
\label{subsec:psnr_eval}
We first evaluate the ability of the normalized 3DGS to reconstruct scenes compared to the original 3DGS formulation.
We evaluate reconstruction quality on two common RGB-D datasets. First, the method was evaluated on Replica~\cite{straub2019replica}, which is a simulated dataset. 
Replica contains sequences of simulated images at 20Hz; these were decimated to 2Hz after which 1 in every 8 retained images was excluded from training for evaluation.
Next, Normalized 3DGS was evaluated on TUM-RGBD~\cite{sturm12tumrgbd}, which is a real-world dataset.
TUM-RGBD is a relatively difficult dataset for accurate 3D reconstruction due to low-resolution images and noisy depth data.
TUM-RGBD sequences were downsampled to achieve an approximate total of 250 images per sequence.
Again, 1 in every 8 images was excluded from training for evaluation.
The reported metrics were only computed on the images excluded from training.

% \iftoggle{abbreviate}{
% Reconstruction results, measured by SSIM and PSNR.
% Additionally, the geometric accuracy of each method is evaluated by measuring the difference between the rendered depth and ground-truth depth.
% For each image excluded from training, a depth image is rendered and compared to the ground truth.
% The Root-Mean-Square (RMS) of the depth error is calculated for each image and then averaged over all images to find the final metric.
% Results are summarized by averaging across each dataset in Table \ref{tab:abbrev_reconstruction}, and comprehensive results are provided in Appendix\ref{app:full_results_abbrev}.
% Across all metrics, Normalized 3DGS approaches the accuracy of standard 3DGS, as shown in Table~\ref{tab:l1_depth_rmse}.
% This is a positive result, since the normalization adds significant complexity to the training process and is the only method allowing risk-aware planning.
% \begin{table}[]
%     \centering
%     \begin{tabular}{c|c}
%          &  \\
%          & 
%     \end{tabular}
%     \caption{Caption}
%     \label{tab:my_label}
% \end{table}
% }{
Visual reconstruction results, measured by SSIM and PSNR~\cite{hore2010psnrssim}, are shown in Table~\ref{tab:ssim_psnr}. 
Experiments indicate that Normalized 3DGS approaches the visual reconstruction quality of standard 3DGS.
This is a positive result, since the normalization adds significant complexity to the training process and is the only method allowing risk-aware planning.


Additionally, the geometric accuracy of each method is evaluated by measuring the difference between the rendered depth and ground-truth depth.
For each image excluded from training, a depth image is rendered and compared to the ground truth.
The Root-Mean-Square (RMS) error is calculated for each image and then averaged over all images to find the final metric.
Similar to SSIM and PSNR results, Normalized 3DGS approaches the accuracy of standard 3DGS, as shown in Table~\ref{tab:l1_depth_rmse}.


\subsection{Collision Probability Evaluation}\label{subsec:collision_evals}
We first evaluate the performance of our constraint representation and compare it against existing methods that plan in radiance fields.
In particular, we compare against \catnips~\cite{chen2023catnips}, which represents the world using a Neural Radiance Field, and \splatnav~\cite{chen2024splatnav}, which represents the world using an un-normalized 3D Gaussian Splat.
Each method's collision representation is shown in Fig.~\ref{fig:collision_comparison}.
The NeRF representation for \catnips was trained using Instant-NGP~\cite{mueller2022instant}, while the \splatnav scene representations were built using the original Gaussian Splatting method~\cite{kerbl20233d}.
We treat each collision detection method as a classifier to determine whether a configuration will result in a collision. 
The performance of each method is measured by evaluating the precision and recall of the collision classifier~\cite{powers2008precrec}.
A True Positive indicates the correct identification of a collision, while a True Negative indicates the correct identification of free space.
 

In each scene, the arm configurations are classified into three categories: Unsafe (in collision), Nearly Safe ($<40$cm to the nearest obstacle), and Safe ($>40$cm to the nearest obstacle). We randomly sample 30 configurations of the arm, which includes 10 configurations from each category to ensure an informative collection of samples.
Since the \catnips and \methodname methods are described for spherical robots, we conduct our experiments by evaluating the collision over the individual spheres that comprise the robot's spherical forward occupancy.
Further, to simplify the comparison with \catnips, we set each sphere to have the radius of the largest sphere in the SFO. 
Finally, \catnips and \splatnav are evaluated using our re-implementations of their respective constraints; as a result, we refer to their respective results as \catnipsstar and \splatnavstar.
Descriptions of the re-implementations are detailed in Appendix \ref{app:impl_details}.

% \iftoggle{abbreviate}
% {
% \begin{figure}
%   \centering
%   \includegraphics[width=0.9\columnwidth]{figures/precision_recall_tro_cropped.pdf}
%   \caption{Treating the collision constraints from \methodname, \catnipsstar, \splatnavstar as a classifiers, where a positive indicates collision and negative indicates no collision, allows evaluating the respective precision-recall curves.}
%   \label{fig:precision_recall}
%   \vspace{-0.25in}
% \end{figure} 
% }{
\begin{figure}
  \centering
  \includegraphics[width=\columnwidth]{figures/precision_recall_tro_cropped.pdf}
  \caption{Treating the collision constraints from \methodname, \catnipsstar, \splatnavstar as a classifiers, where a positive indicates collision and negative indicates no collision, allows evaluating the respective precision-recall curves.}
  \label{fig:precision_recall}
\end{figure}
% }
\input{tables/planning_results}



We calculate the Precision-Recall values at various thresholds corresponding to the allowable collision risk.
\methodname, \catnips, and \splatnav each express this maximum allowable risk differently.
For \methodname, we vary the parameters $\alpha$ and $\beta$, in the range of (0,1), as discussed in Section~\ref{subsec:approach_collision}.
For \catnips, we vary the collision probability $\sigma$ and the maximum number of auxiliary particles that may exist in the robot's volume, denoted $N^{max}_{aux}$. 
We refer the interested reader to~\cite{chen2023catnips} for a detailed explanation of these parameters.
In our experiments, $N_{aux}^{max}$ is set to $\{1,5,10\}$ while using $V_{aux}$ as $10^{-6}$, and $\sigma$ is varied in the range of (0,1). 
Finally, \splatnav deterministically checks whether the robot collides with the 99\% confidence ellipsoids, meaning the method does not emit a risk parameter.
Instead, we evaluate the method across several level sets of the Gaussian functions, ranging from the 1-sigma ellipsoid to the 10-sigma ellipsoid.

We report Precision-Recall curves in Fig.~\ref{fig:precision_recall}.
\catnipsstar achieves a high precision, indicating that most of the detected collisions were true collisions.
However, the comparatively low recall indicates that unsafe configurations were classified as safe.
\splatnavstar achieves higher recall, indicating that the method is more conservative and will result in fewer collisions.
However, the lower precision indicates the presence of false positives, which would cause a motion planner to behave overly conservatively.
The \methodname constraint achieves higher precision and recall than either \splatnavstar or \catnipsstar.
Further, Fig.~\ref{fig:precision_recall} shows that the thresholds $\alpha$ and $\beta$ in \methodname allow for significant control of the behavior of the constraint, ranging from highly aggressive near the left to more conservative on the right.

==> sections/YY_symbols.tex <==
\section*{List of Symbols}
\subsection*{Nomenclature}
\begin{itemize}
    \item Gaussian splat is a noun
    \item Gaussian splatting is a verb
    \item Splan is a noun
    \item Spanning is a verb
\end{itemize}

\subsection*{Colors}
\begin{itemize}
    \item Purple - reachable set
    \item Red - obstacles
    \item Green - goal configuration
\end{itemize}

\subsection*{Generic Mathematical Symbols}
\begin{itemize}
%   \item $\lambda_j$: indeterminants
  \item $n$: generic constant
  \item $\mathbb{N}$: natural numbers
  \item $\mathbb{R}^n$: reals 
%   \item $S_i(t)$: sliced reachable set
  \item $X$: a general set and/or metric space
\end{itemize}

\subsection*{Zonotope Symbols}
\begin{itemize}
    \item $Z$: generic zonotope
    \item $Z_1$: generic zonotope
    \item $Z_2$: generic zonotope
    \item $Z_1^g$: a zonotope with a center at the origin and the same generators of a zonotope, $Z_1$
    \item $Z_2^g$: a zonotope with a center at the origin and the same generators of a zonotope, $Z_2$
    \item $\beta_i$: zonotope indeterminants
    \item $\beta_{\forall}$: all indeterminants of a zonotope
    \item $c$: zonotope center
    \item $g_i$: ith zonotope generator
    \item $g_{\forall}$: all generators of a zonotope
    \item $\pzgi$: ith PZ coefficient (aka generator)
    \item $G_i$:  ith generator matrix of Matrix zonotope 
    \item $\nhj$: number of halfspaces of $\Pj$
    \item $M$: matrix zonotope
    \item $\pzn$: number of PZ generators
    \item $p_1$: generic point inside poly zonotope
    \item $p_2$: generic point inside poly zonotope
    \item $\pz{P_1}$: generic polynomial zonotope
    \item $\pz{P_2}$: generic polynomial zonotope
    \item $\Pj$: convexhull of $j$-th link's buffered FRS
    \item $\pz{R_{j-1}^j}$: poly zonotope representation of orientation of frame $j-1$ \textit{wrt} frame j
    \item $\pzv$: indeterminant for polynomial zonotope
    \item $\pzgi$: ith PZ coefficient (aka generator)
    \item $\sigma$: coefficient to be sliced/evaluated
\end{itemize}

\subsection*{Coordinate frames and Transformations}
\begin{itemize}
    \item $C$: camera with ROS convention (x right, y down, z out)
    \item $\homtrans_{j}^{j-1}(\qj)$
    \item $i$: standard notation for indicating time step
    \item $I$: Image plane frame (u,v) 
    \item $j$: standard notation for indicating joint frame
    \item $\nd$: dimension of the
    \item $p_j$: position of frame $j$ relative to frame $0$
    \item $p_{j-1,j}^j$: position of frame $j$ wrt frame $j-1$ expressed in frame $j$
    \item $Q$: configuration space
    \item $R_{j-1}^j$: orientation of frame $j-1$ \textit{wrt} frame $j$
    \item $R_j(q(t))$: orientation of frame $j$ \textit{wrt} frame $0$
    \item $t$: time
    \item $^Wx$: point $x$ represented in the world frame $W$ \jon{This notation isn't consistent with the other symbols}
    \item $W$: world frame
    \item $W_s$ workspace frame of the robot \seth{Do we need both world and workspace?} 
    \jon{The workspace describes all points reachable by the robot. The distinction between world and workspace is relevant if we want to discuss culling gaussians that are always too far away.}
    \item $\omega_i^j$: frame $j$ angular velocity wrt frame $j$
    \item $\dot{\omega}_j^j$: frame $j$ angular acceleration wrt frame $j$
\end{itemize}

\subsection*{Trajectory Symbols}
\begin{itemize}
    \item $\kscale$: scale for $k$ interval
    \item $i$: time index
    \item $k$: trajectory parameter
    \item $K$: space of trajectory parameters
    \item $\nt$: number of time steps
    \item $j\in\Nq$: $j\in\{1,\cdots,\nq\}$
    \item $i\in\Nt$: $i\in\{1,\cdots,\nt\}$
    \item $h\in\Nhj$: $h\in\{1,\cdots,\nhj\}$
    \item $t$: time
    \item $t_i$: indexed time
    \item $T$: time horizon
\end{itemize}

\subsection*{SFO symbols}
\begin{itemize}
    \item 
    \item $c_{j,m}(k)$: The center of the m$^{th}$ sphere on the $j^{th}$ link
    \item $j$: index for specifying joint/link
    \item $\ell_{j,m}(k)$:
    \item $r_{j,m}(k)$: The radius of the m$^{th}$ sphere on the $j^{th}$ link
    \item $j$: index for specifying link
    \item $t$: index for specifying time interval
    \item $m \in \{1, 2\}$: index for specifying cap sphere of links, or the joint spheres in the Spherical Joint Occupancy. $1$ is closer to the base in the kinematic tree. $2$ is closer to the end effector in the kinematic tree.
    \item $i$: index for specifying the sphere on the link in the Spherical Link Occupancy
    \item $\mathbf{C}_{t,j,m}$: PZ for the center of joint sphere $m$ in the Joint Spherical Occupancy for link $j$ at the $t^{th}$ time interval.
    \item $c_{t,j,m}$: Some point center of joint sphere $m$ in the Joint Spherical Occupancy for link $j$ at the $t^{th}$ time interval, sliced from $\mathbf{C}_{t,j,m}$.
    \item $r_{t,j,m}$: Radius of the respective joint sphere.
    \item $S_{t,j,m} = (c_{t,j,m}, r_{t,j,m})$: Joint spheres for link $j$ at time interval $t$.
    \item $\mathbf{S}_{t,j,m} = (\mathbf{C}_{t,j,m}, r_{t,j,m})$: Spherical Joint Occupancy for joint $m$ related to link $j$ at time interval $t$.
    \item $S_{t,j,2} = S_{t,j+1,1}$ and $\mathbf{S}_{t,j,2} = \mathbf{S}_{t,j+1,1}$
    \item $\bar{c}_{t,j,\ell}(k)$: Center of the $i^{\text{th}}$ sphere on the $j^{\text{th}}$ link for the $t^{\text{th}}$ time interval in the Spherical Link Occupancy
    \item $\bar{r}_{t,j,\ell}(k)$: Radius of the $i^{\text{th}}$ sphere on the $j^{\text{th}}$ link for the $t^{\text{th}}$ time interval in the Spherical Link Occupancy
    \item $\bar{S}_{t,j,\ell} = (\bar{c}_{t,j,\ell}, \bar{r}_{t,j,\ell})$: Joint spheres for link $j$ at time interval $t$.
\end{itemize}

\subsection*{3D Scene representation Symbols}
\begin{itemize}
    \item $C_a^b[\ray]$: random event describing the collision along a ray $\ray$ from $a$ to $b$
    \item $\ray(t)$: ray
    \item $\sigma(t)$: density
    \item $\transmit$: Transmittance 
    \item \jon{A bunch of probabilities need to be defined}
\end{itemize}

\newpage
